Who Should Teach? Confidence-Aware Dual-Teacher Learning for Few-Shot Node Classification on Text-Attributed Graphs

Text-Attributed Graphs (TAGs) integrate graph structures and node-associated textual attributes, and recent studies have increasingly leveraged Large Language Models (LLMs) to improve TAG learning in few-shot settings. However, existing approaches typically utilize LLM-derived information uniformly across all nodes, despite substantial variations in its reliability, while also incurring considerable monetary costs. We argue that the most appropriate source of supervision may differ across nodes, as Graph Neural Networks (GNNs) and LLMs exhibit complementary strengths in exploiting structural and semantic information, respectively. To this end, we propose CoTeach, a Confidence-aware dual-teacher learning framework that dynamically selects the more reliable teacher for each node. Experimental results demonstrate that CoTeach consistently improves few-shot node classification performance while reducing unnecessary LLM utilization and associated monetary costs.

==> Link/Tabs/pr.tex <==
\begin{table*}[t]
\centering
\footnotesize
\caption{Illustrative example of the prompt used by the LLM teacher.}
\label{tab_p}
\vspace{-4mm}
\def\arraystretch{1.2}
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{p{2.8cm}p{15.5cm}}
\toprule
\textbf{Component} & \textbf{Content}
\\ \midrule

\textbf{System}
&
You are a careful classifier for wiki articles.
\\

\textbf{Task}
&
Read the title and abstract of a target article and estimate a probability distribution over candidate categories.
\\

\textbf{Candidate Categories}
&
Computational Linguistics, Databases, Operating Systems, Computer Architecture, Computer Security,
Internet Protocols, Computer File Systems, Distributed Computing Architecture,
Web Technology, Programming Language Topics.
\\

\textbf{Target Paper}
&
\textbf{Title:}
\textit{datasource.datasource datasource name given connection set database server name commonly used creating query database ...}
\\
&
\textbf{Abstract:}
\textit{datasource object represents an alternative to DriverManager, provides database connections,
supports JNDI registration, connection pooling, distributed transactions, and JDBC-based access to data sources ...}
\\

\textbf{Generation Rules}
&
(1) \texttt{predicted\_label} must exactly match one candidate category.
(2) \texttt{class\_probs} must contain all candidate categories exactly once.
(3) Probabilities must be within $[0,1]$ and sum to 1.0.
(4) Only assign very high confidence when strong evidence exists.
(5) Do not generate explanations or additional text.
\\

\textbf{Output Format}
&
\texttt{predicted\_label: <category>}
\\
&
\texttt{class\_probs: \{category\_1:p\_1, category\_2:p\_2, ..., category\_n:p\_n\}}
\\

\textbf{Example Response}
&
\texttt{predicted\_label: Databases}
\\
&
\texttt{class\_probs:}
\\
&
\texttt{\{}
\\
&
\texttt{\ \ Databases: 0.60,}
\\
&
\texttt{\ \ Computer Security: 0.20,}
\\
&
\texttt{\ \ Computer File Systems: 0.10,}
\\
&
\texttt{\ \ Programming Language Topics: 0.10,}
\\
&
\texttt{\ \ Computational Linguistics: 0.00,}
\\
&
\texttt{\ \ Operating Systems: 0.00,}
\\
&
\texttt{\ \ Computer Architecture: 0.00,}
\\
&
\texttt{\ \ Internet Protocols: 0.00,}
\\
&
\texttt{\ \ Distributed Computing Architecture: 0.00,}
\\
&
\texttt{\ \ Web Technology: 0.00}
\\
&
\texttt{\}}
\\

\bottomrule
\end{tabular}
}
\vspace{-5mm}
\end{table*}
